Locally Self-Adjusting Skip Graphs

We present a distributed self-adjusting algorithm for skip graphs that minimizes the average routing costs between arbitrary communication pairs by performing topological adaptation to the communication pattern. Our algorithm is fully decentralized, conforms to the $\mathcal{CONGEST}$ model (i.e. uses $O(\log n)$ bit messages), and requires $O(\log n)$ bits of memory for each node, where $n$ is the total number of nodes. Upon each communication request, our algorithm first establishes communication by using the standard skip graph routing, and then locally and partially reconstructs the skip graph topology to perform topological adaptation. We propose a computational model for such algorithms, as well as a yardstick (working set property) to evaluate them. Our working set property can also be used to evaluate self-adjusting algorithms for other graph classes where multiple tree-like subgraphs overlap (e.g. hypercube networks). We derive a lower bound of the amortized routing cost for any algorithm that follows our model and serves an unknown sequence of communication requests. We show that the routing cost of our algorithm is at most a constant factor more than the amortized routing cost of any algorithm conforming to our computational model. We also show that the expected transformation cost for our algorithm is at most a logarithmic factor more than the amortized routing cost of any algorithm conforming to our computational model.

==> dsg_backup_detail.tex <==
\section{Dynamic Skip Graphs (DSG)} \label{sec:dsg}
Upon a communication request, our proposed algorithm \textsf{DSG} establishes communication using the standard skip graph routing, followed by locally performed topological adaptation conforming to the skip graph model.
%
Let $H_t$ be the height of the skip graph at time $t$, where height is the number of levels.
%
Our algorithm requires a node to have an unique identifier which we assume to be a number (can be ip address).
%
It is required that any two unique identifiers differ by at least 1.
%
Our algorithm also requires every node to hold $H_t$ bits to store its membership vector.
%
In addition, each node stores $H_t$ sets (1 set for each level) of two different variables: {\em timestamp} and {\em group-id}.
%
A node is a member of a group at each level, and the group-id is an identifier that represents a group.
%
The timestamp associated with a level is the time when the node is considered to be active at that level. The timestamp is used by our algorithm to identify how attached a node is with its group at some level.
%
Each node also stores a number (between 0 and $H_t$) referred to as \emph{group-base}.
%
the group-base for a node is the highest level at which the node's group contains the highest number of nodes among all the groups the node belongs to.
%


For node $i$ and level $j$, we use the notations $V^i_j$, $T^i_j$, and $G^i_j$ to denote the stored membership vector bit, timestamp, and group-id, respectively. We use the notation $B_x$ to denote the group-base of node $x$. Initially, all timestamps are set to zero, all group-ids are set to the corresponding node's identifier, and the group-base for all nodes are set to the height of the skip graph. Every node also holds a constant $C$ (common to all nodes) which must be greater than any possible height $H_t$. Note that, according to our model the height must be $O(\log n)$.

\begin{figure}[htpb]

    \begin{subfigure}[b]{0.4\textwidth}
        
        \includegraphics[width=1\textwidth]{./figs/ex_com_g.pdf}
        \caption{A communication graph $G$}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.75\textwidth}
        
        \includegraphics[width=1\textwidth]{./figs/ex_tree1.pdf}
        \caption{Skip graph at time 7, $S_7$.}
    \end{subfigure}
    
    
    \begin{subfigure}[b]{0.75\textwidth}
        
        \includegraphics[width=1\textwidth]{./figs/ex_tree2.pdf}
        \caption{Skip graph at time 8, $S_8$.}
    \end{subfigure}
    
    
    
    \caption{For the access pattern shown in (a), the working set number for the last communication between $u$ and $v$ is 5, as the the number of distinct nodes in $G$ that has a path from either $u$ or $v$ is 5 (e,a,k,u and v).}
    \label{fig:wset}
\end{figure}







For a communication request from node $u$ to node $v$, let $\alpha$ be the highest common level of current skip graph with a linked list containing both $u$ and $v$. Let $l_\alpha$ denotes that linked list, then $u,v \in l_\alpha$, and $l_\alpha \in L_\alpha$, where $L_\alpha$ denotes the set of linked lists at level $\alpha$.
{\color{red}Note that every linked list in the skip graph is mapped to an unique node in the equivalent binary search tree as shown in figure \ref{fig:sg_to_tree}}.
Let $t$ be the time when the request is originated, and $S_t$ be the skip graph at time $t$. Table \ref{tab:notation} lists the frequently used notations.

\begin{table}[htbp]
\scriptsize
\centering
\begin{tabular}{|c|l|}
\hline
\textbf{Notation} & \textbf{Description} \\[1ex]
%heading
\hline
$m(x)$ & membership vector of node x \\
$V^i_j$ & node i's membership vector bit for level j \\
$T^i_j$ & timestamp for node i at level j \\
$G^i_j$ & group-id for node i at level j\\
$B_x$ & group-base of node x \\
$l_a$ & a linked list at level a  \\
$S_t$ & skip graph at time t\\
\hline
\end{tabular}
\caption{Notations}
\label{tab:notation}
\end{table}


For the ease of referencing, we divide our algorithm into 13 steps. Upon a communication request from node $u$ to node $v$, our algorithm \textsf{DSG} works as follows:

\textbf{Step 1.} communication is established using the standard skip graph routing algorithm. When the routing is done, $v$ records $\alpha$ and share $\alpha$ with $u$. Then both nodes $u$ and $v$ broadcast a transformation notification to all nodes in $l_\alpha$. The notification message includes all $H_t$ timestamps, group-ids and membership vectors of nodes $u$ and $v$. The notification message also includes the group-bases for both nodes $u$ and $v$.





\textbf{Step 2.} All nodes  $x \in l_\alpha$ assign a priority $P(x)$ by using following priority-rules:

\begin{enumerate}

\item[P1:] (Rule for communicating nodes). Node $u$ and $v$ sets $\infty$ as their priority. In other words, set $P(u) = P(v) = \infty$.

\item[P2:] (Rule for nodes in the same group of either communicating nodes at level $\alpha$). All nodes $x \in l_\alpha, x \neq u, x \neq v, G^x_\alpha = G^u_\alpha$ assign their priority $P(x) = T^x_c$ where $c$ is the highest level such that $G^x_c = G^u_c$. Similarly, all nodes $x \in l_\alpha, x \neq u, x \neq v, G^x_\alpha = G^v_\alpha$ assign $P(x) = T^x_c$ where $c$ is the highest level such that $G^x_c = G^v_c$.


\item[P3:] (Rule for other nodes). All nodes $x \in l_\alpha, x \neq u, x \neq v, G^x_\alpha \neq G^u_\alpha$ (i.e. neither in $u$'s nor in $v$'s group at level $\alpha$) set \\
$P(x) = - \sum \limits_{i = \alpha}^{H_t} 2^{(C - i)} G^x_i $

\end{enumerate}


\textbf{Step 3.} All nodes $x \in l_\alpha$ with $G^x_\alpha = G^u_\alpha$ or $G^x_\alpha = G^v_\alpha$  set $G^x_\alpha = u$; in other words $u$'s group at level $\alpha$ merges with $v$'s group at that level by setting the same identifier as their group-ids.



\textbf{Step 4.} Transformation begins at level $\alpha + 1$ and recursively continues at upper levels. Only the nodes in linked list $l_\alpha$ take part in the transformation. For the remaining paper, we write $d$ to refer the current level of transformation and $l_{d-1}$ to refer the linked list that is involved in the transformation. Initially $d=\alpha + 1$ and $l_{d-1}=l_\alpha$. We find an approximate median priority to decide whether a node should go to the 0-subgraph or to the 1-subgraph (i.e. determine new membership vector bit $V^x_{\alpha+1}$) in the new skip graph $S_{t+1}$. We propose an approximate median finding algorithm (\textsf{AMF}) for skip graphs to find the approximate median in expected $O(\log_a n)$ rounds, where $a$ is a constant. The algorithm \textsf{AMF} is described in section \ref{sec:amf}. For now let us consider \textsf{AMF} as a black box that finds an approximate median priority and broadcasts it to all nodes in linked list $l_{d-1}$.

\textbf{Step 5.} Let the approximate median priority be $M$. If $M$ is negative, all nodes $x$ receiving $M$ check the following condition:

\begin{equation} \label{eq:gr_split}
- 2^{(C-(d-1))} \cdot G^x_{d-1}  \geq M \geq - 2^{(C-(d-1))} \cdot ( G^x_{d-1} + 1)
\end{equation}

Let $g_s$ be the group such that all nodes $x \in g_s$ finds the condition in \ref{eq:gr_split} true. As the approximate median priority is used by nodes to decide whether to move to 0-subgraph or 1-subgraph at level $d$, group $g_s$ (if exists) may get split at level $d$ as its nodes may move to different subgraphs. Given that $m$ is negative, the priority rule P3 confirms that group $g_s$ contains neither $u$ nor $v$. Let $(x,y)$ be any node pair in group $g_s$, $d_{S_{t+1}}(x,y)$ be the routing distance between $x$ and $y$ after transformation, and $t_i (x,y)$ be the working set number for $(x,y)$ pair at time $t+1$; our goal is to ensure that $d_{S_{t+1}}(x,y) = O(\log t_i (x,y))$ in skip graph $S_{t+1}$. We claim that this property will be violated if the group $g_s$ is split at level $d$ since it will increase the distance between some node pairs $(x,y)$.

All nodes $x \in l_d$ reuse the balanced skip list created by algorithm \textsf{AMF} to compute the size of following four sets:

\begin{itemize}

\item $L_{low} = \{x \in l_d | P(x) \leq M\}$
\item $L_{high} = \{x \in l_d | P(x) > M\}$
\item $g_{low} = \{x \in g_s | P(x) \leq M\}$
\item $g_{high} = \{x \in g_s | P(x) > M\}$

\end{itemize}


To compute these sizes, all nodes $x \in l_{d-1}$ form a vector of 4 counts where each count is associated with one of the above sets. The initial value for each count is either 0 or 1 depending upon $P(x)$ and node's membership in $g_s$. We refer this vector as the \emph{count vector}. Now, each node $x \in l_{d-1}$ such that $x$ does not step up at level $d$ in the balanced skip list forwards its count vector to the left neighbor in linked list $l_{d-1}$. Any node $x \in l_{d-1}$ receiving a vector from the right neighbor adds its own vector with the received vector, and forwards the resultant vector to the left neighbor in linked list $l_{d-1}$ only if $x$ does not step up to level $d$. {\color{red} This ensures that the counts for all nodes are summed up and linearly forwarded to their nearest right neighbor that steps up to level $d$}. Similar linear forwarding takes place recursively at all upper levels. As a result, the right most node in $l_{d-1}$ (also the root node of the skip list) receives the finals counts for all nodes in the skip list. The count vector with the final counts are broadcasted to all nodes $x \in l_{d-1}$.


\textbf{Step 6.} Each node $x \in l_{d-1}$ decides whether to move to the 0-subgraph (by setting the membership vector bit $V^x_d = 0$) or to the 1-subgraph at level $d$. If the approximate median priority $M \geq 0$, any node $x \in l_{d-1}$ with $P(x) \leq M$ moves to the 0-sublist and any node $x \in l_{d-1}$ with $P(x) > M$ moves to the 1-sublist. Due to the priority rules P1, P2 and P3, this ensures that communicating nodes $u$ and $v$ always move to the 0-subgraph. However, if $M < 0$, nodes decide which sublist to move to as follows:

\begin{itemize}

\item[--] If $(g_{low} + g_{high}) > \frac{2}{3} (L_{low} + L_{high})$
    \begin{itemize}
    \item any node $x \in l_{d-1}$ moves to the 0-subgraph if $P(x) \leq M$; $x$ moves to the 1-subgraph otherwise.
    \end{itemize}

\item[--] If $(g_{low} + g_{high}) < \frac{1}{3} (L_{low} + L_{high})$

    \begin{itemize}
    \item any node $x$ such that $x \in l_{d-1} \text{ and } x \not \in g_s$ moves to the 0-subgraph if $P(x) \leq M$; $x$ moves to the 1-subgraph otherwise.
    \item any node $x \in g_s$ moves to the 0-subgraph if $L_{low} < L_{high}$; $x$ moves to the 1-subgraph otherwise.
    \end{itemize}

\item[--] If $\frac{1}{3} (L_{low} + L_{high}) \leq (g_{low} + g_{high}) \leq \frac{2}{3} (L_{low} + L_{high})$
    \begin{itemize}
    \item any node $x$ such that $x \in l_{d-1} \text{ and } x \not \in g_s$ moves to the 0-subgraph.
    \item any node $x \in g_s$ moves to the 1-subgraph.
    \end{itemize}


\end{itemize}


Therefore, two new linked lists are formed at level $d$. To find the left and right neighbors at level $d$, nodes linearly search for neighbors at level $d-1$. Because of the a-balance property, it is guaranteed that a node finds both of its left and right neighbors in at most $a$ rounds unless the node is an end-node of the new linked list.


\textbf{Step 7.} Each node $x \in l_{d-1}$ checks if the a-balance property is being violated at level $d$ by the rearrangement of nodes. The balanced skip list created by \textsf{AMF} is reused to check if any consecutive $a$ nodes at level $d-1$ have moved to the same subgraph at level $d$. All nodes in the skip list at level $d$ check the new membership vector bit of $a$ nearby nodes at level $d-1$ in both sides and share this information with both neighbors of the skip list at level $d$ to detect chains. If a chain of size $a$ or longer is detected, a dummy node is placed in the sibling subgraph at level $d$ to break the chain. A dummy node is a logical node which requires $O(\log n)$ links and a key. A dummy node does not hold any data. When a dummy node is placed to break a chain, the key is picked by checking the key of a neighbor of the dummy node at level $d$ to make sure all keys remain sorted at the base level -- hence the skip graph property remains intact in $S_{t+1}$. A dummy node destroys itself when it receives a transformation notification by a future \textsf{DSG} call. While being destroyed, a dummy node simply links its left and right neighbors at all levels and deletes itself. The sole purpose of dummy nodes is to ensure that a-balance property is always preserved. To implement dummy nodes, all regular nodes must have the ability to hold extra $O(\log n)$ links. Since a dummy node does not hold any data, it requires minimal computational resource and memory. It is important to note that a dummy node is logically separated from the host node, and only used for routing purpose.

\textbf{Step 8.} Each node $x \in l_{d-1}$ checks if nodes $u$ and $v$ belong to their own linked list at level $d$ by checking the following condition.

\begin{equation} \label{eq:uv_check}
V^x_{\alpha+1} = V^x_{\alpha + 2} = ... = V^x_d = 0
\end{equation}


If a node finds the condition \label{eq:uv_check} to be
true, a linked list (0-sublist) created by the rearrangement must contain nodes $u$ and $v$. In this case, all such nodes $x$ set their group-id $G^x_d = u$.

On the other hand, if the condition \label{eq:uv_check} is found to be false for any node, it checks if its group at level $d$ is getting split due to the rearrangement. A group without communicating nodes $u$ and $v$ can split at level $d$ only if the group is $g_s$.
%Since the priorities for these nodes are set by using the priority rule P3, the key idea here is that group-ids are unique node identifiers and two group-ids differ by at least 1.
In case of such a split, the identifier of the left-most node in a split group is used as the new group-id. Observe that it is easy for the left-most node to detect itself as it does not find a neighbor at left. The balanced skip list structure created by algorithm \textsf{AMF} is then used to propagate the new group-id to all nodes of the group. The left-most node first sends its identifier to the head node of the balanced skip list, and then the identifier is broadcasted to all nodes at the base level of the skip list. The balanced skip list is destroyed once the new group-id is sent to all members of the group. Each node $x \in l_{d-1}$ that finds condition \label{eq:uv_check} false also reassigns their priority by setting $P(x) = - \sum \limits_{i = d-1}^{H_t} 2^{(C - i)} G^x_i $. We refer this as the priority rule P4.


\textbf{Step 9.} Above steps 2-8 execute recursively and parallelly for each newly created linked list that contains more than one node for levels $d = \alpha+1, \alpha +2, \dots, H_{t+1}$. This recursive procedure ends when all nodes become singleton and the only member in its linked list. Clearly this ensures that node $u$ and $v$ get connected directly, and all nodes $x \in l_\alpha$ finds their new and complete membership vectors.



\textbf{Step 10.} Nodes update their group-ids for levels below $\alpha$ at this step. Recall that after $u$'s group merges with $v$'s group at level $\alpha$, the new group id is $u$. Each node $x \in l_\alpha$ with $G^x_\alpha = u$  initializes a vector $G_{lower}$ as follows:


\[
    G_{lower}=
\begin{cases}
    [G^u_{0}, G^u_{1}, \dots,  G^u_{\alpha-1}],& \text{if } B_u \leq B_v\\
    [G^v_{0}, G^v_{1}, \dots,  G^v_{\alpha-1}],& \text{otherwise}
\end{cases}
\]


If $\min (B_u, B_v) < \alpha$, node $u$ broadcasts a message  \\ $\big \langle G_{lower}, \min (B_u, B_v) , G^u_{\max (B_u, B_v)} , G^v_{\max (B_u, B_v)} \big \rangle$ to all nodes $y \in l_{\max (B_u, B_v)}$ such that $u,v \in l_{\max (B_u, B_v)}$. Each such node $y$ with $G^y_{\max (B_u, B_v)} = G^u_{\max (B_u, B_v)}$ or $G^y_{\max (B_u, B_v)} = G^v_{\max (B_u, B_v)}$ updates their group-base level $B_y = \min (B_u, B_v)$ and sets $G^y_i = G_{lower}[i]$ for $ i = 0, 1, \dots \alpha - 1$.

Regardless of the outcome of the comparison $\min (B_u, B_v) < \alpha$, each node $x \in l_\alpha$ with $G^x_\alpha = u$ sets $G^x_i = G_{lower}[i]$ for $ i = 0, 1, \dots \alpha - 1$.





\textbf{Step 11.} Each node $x \in l_\alpha$ updates its group-base level $B_x$ as follows:

\begin{itemize}

\item[--] If $x$'s group at any level $d$ ($d \geq \alpha$) splits into 2 subgroups due to transformation, and if $B_x = d$, $x$ sets $B_x = B_x - 1$.

\item[--] Let $d$ be the lowest level at which $x$'s group splits due to transformation. if $B_x = \alpha$ and $d > \alpha+1$, $x$ sets $B_x = d - 1$.

\end{itemize}






\textbf{Step 12.} Each node $x \in l_\alpha$ updates its timestamps by using the following timestamp-rules (executed in the order given below):

\begin{enumerate}

\item[T1:]  Node $u$ and $v$ set all $T^u_i = T^v_i = t$ ($t$ is the timestamp for the current communication request) for $i = j, j+1, ... , H_{t+1}$ where $j$ is the lowest level s.t. $G^u_j = G^u_\alpha$.  Node $u$ and $v$ set $T^u_i = T^v_i = max(T^u_i, T^v_i)$ for $i = 1,2,...,j-1$.

\item[T2:] Let $x$ be a node s.t. $x \neq u, x \neq v, x \in l_\alpha$ with $G^x_\alpha = G^u_\alpha$ before transformation. Let $c^\prime$ is the longest common postfix between $m(u)$ and $m(x)$ in $S_t$ and $c^{\prime \prime}$ be the longest common postfix between $m(u)$ and $m(x)$ in $S_{t+1}$. If $c^\prime > c^{\prime \prime}$, each such node $x$ sets $T^x_i = T^x_{c^\prime}$ for all $i =  c^\prime - 1,  c^\prime - 2, ...  c^{\prime \prime}$. Similarly, each $x$, $x \neq u, x \neq v, x \in l_\alpha$ with $G^x_\alpha = G^v_\alpha$ at time $t$ (before transformation), updates their timestamps w.r.t. node $v$. Note that, $T^x_{c^\prime}$ is the priority $P(x)$ computed by P2.

\item[T3:]  Each node $x$ that initialized or received $G_{lower}$ at step 10 finds the lowest level $d$ such that $T^x_{d+1} = 0$. If such a $d$ exists and if $d > B_x$, node $x$ sets $T^x_d = T^x_{d-1} = \dots = T^x_{B_y} = T^x_{d+1}$.


\item[T4:] Let $x$ be a node, $x \in l_\alpha$ and $x$ belongs to a group $g$ at level $d$, $d \geq \alpha$, such that $g$ splits into two subgroups at level $d+1$. Each node $x$ sets $T^x_d = T^x_{d+1}$ only if $T^x_d = 0$.


\end{enumerate}







\textbf{Step 13.} All nodes $x \in l_\alpha$ independently set themselves free for the next communication or transformation.

A summary of the algorithm \textsf{DSG} is presented in algorithm \ref{alg:DSG}.



\textbf{Node addition and removal.} Nodes can be added or removed by using standard node addition or removal procedures for skip graphs. When a node is added, the new node needs to initialize its variables (group-ids, timestamps and group-base levels) with the default values. Following a node addition, the new node checks if the a-balance property is violated due to the node addition. Following a node deletion. a neighbor of the deleted node from each level checks if the a-balance property is violated due to node deletion. In case of a violation, the node initiates appropriate dummy node.






\begin{algorithm}[]
\label{alg:DSG}
\DontPrintSemicolon

%\KwData{$G=(X,U)$ such that $G^{tc}$ is an order.}
%\KwResult{$G’=(X,V)$ with $V\subseteq U$ such that $G’^{tc}$ is an interval order.}
\caption{Dynamic Skip Graph \textsf{DSG}\label{DSG} (summary)}

Upon request $(u,v)$ in $S_t$, establish the communication by using standard skip graph routing and find $\alpha$. Broadcast the membership vector, timestamps $T^u_d$, $T^v_d$, group-ids $G^u_d$, $G^v_d$, and group-base levels $B_u$, $B_v$, where $d = \alpha, \alpha+1, ..., H_t$, to all nodes in $l_\alpha$.
\;
Each node $x \in l_\alpha$ computes their priority $P(x)$ using the using priority-rules P1, P2 and P3.
\;
Node $u$'s group at level $\alpha$ merges with node $v$'s group at level $\alpha$ by setting $G^x_\alpha = u$ for each group member $x$.
\;
Let $d = \alpha + 1$ and linked list $l_{d-1} = l_\alpha$. Compute the approximate median priority $M$ by using the algorithm \textsf{AMF}.
\;
Compute $|L_{low}|$, $|L_{high}|$, $|g_{low}|$ and $|g_{high}|$ using the balanced skip list formed by \textsf{AMF} if the condition in \ref{eq:gr_split} is true.
\;
Determine the membership vector bit $V^x_d$ by using $P(x)$, $M$, $|L_{low}|$, $|L_{high}|$, $|g_{low}|$ and $|g_{high}|$.
\;
Reuse the balanced skip list formed by \textsf{AMF} to check if a-balance property is being violated by the rearrangement. If yes, put a dummy node to break the chain violating the a-balance property.
\;
If a group at level $d$ is split into two subgraphs (because of step 6), find new (level $d$) group-id for the split group that moved to the 1-subgraph, and broadcast the new group-id by using the balanced skip list formed by \textsf{AMF}. Each $x$ in that group updates its $G^x_d$ with the new group-id. However, if the linked list formed by nodes that moved to 0-subgraph contains node $u$ and $v$, nodes $x$ set  $G^x_d = u$. Each node $x$ also updates their priorities ($P(x)$) using priority-rule P4 when applicable. Destroy the balanced skip list formed by \textsf{AMF}.
\;
Repeat steps 2 to 8 recursively and parallelly for all newly formed linked lists ($l_{d-1}$) that contains at least 2 nodes.
\;
Update group-ids for levels below $\alpha$ for appropriate nodes.
\;
Update group-base levels for the appropriate nodes.
\;
Update timestamps using timestamps-rules T1-T4.
\;
Independently set nodes ($x \in l_\alpha$) free for next communication.
\;



\end{algorithm}













%###################################
%           section ends here
%#################################

\iffalse


\item[T3:]  After $u$'s group merges with $v$'s group at level $\alpha$, all nodes $x \in l_\alpha$ with $G^x_\alpha = G^u_\alpha$ remember the level at which they received the first positive approximate median priority. According to the rules that are used to set priorities, obviously the merged group will split in subgraphs by a positive approximate median priority. Let the first positive approximate median priority is received at level $c$, then all nodes $x$ with $G^x_\alpha = G^u_\alpha, x \neq u, x \neq v$ checks if there exists a level $d, 1 \leq d \leq \alpha$ s.t. $G^u_d = G^v_d$. If such a $d$ exists, node $x$ finds the lowest level $b$ such that $T^x_b \neq 0$ ($b \geq \alpha$). If such a $b$ exists, node $x$ sets $T^x_c =T^x_{c+1} = ... = T^x_{b - 1} = T^x_b$.


\section{Improving Routing with Allowing Simultaneous Two Searches} \label{sec:dsgds}

A group-base is the base level of a group. As our algorithm \textsf{DSG} merges groups when two nodes from two different groups communicate, it is possible that an uninvolved group gets partitioned into two subgroups due to reconstruction of the transformed skip graph. This may increase distance between two nodes in a group. We handle this problem by using the variable group-base for each of the levels.

Our algorithm \textsf{DSG} works as follows: upon a communication request from node $u$ to node $v$, communication is established as node $u$ invokes the subroutine \textsf{ROUTING} ($u$, $v$, $0$).




Each node $x \in l_\alpha$ with $G^x_\alpha =  G^u_\alpha$ checks if there exists a level $d, 1 \leq d \leq \alpha$ s.t. $G^u_d = G^v_d$. If no such $d$ exists, each node $x \in l_\alpha$ with $G^x_\alpha =  G^u_\alpha$ sets $G^x_0 = G^x_1 = ... = G^x_\alpha = G^u_\alpha$. If $d$ exists, each node $x \in l_\alpha$ with $G^x_\alpha =  G^u_\alpha$ sets $G^x_i = G^u_i$ for $i = d+1, d+2, ..., \alpha$.

Nodes receiving an approximate median priority that splits their group at level $d$ update their group-bases by using the following group-base-rule:

\begin{enumerate}

\item[B1:] Each node $x \in l_\alpha$ with $G^x_\alpha \neq G^u_\alpha$ checks if this is the first time in this transformation node's group is getting split. If the first time, then simply remember the level $d$ by setting $prevd = d$ (suppose $prevd$ is a local variable). If not the first time and if $(d - prevd) > 1$, node $x$ sets $L^x_d = prevd$.

\end{enumerate}



\begin{algorithm}[]
\label{alg:routing}
\DontPrintSemicolon

%\KwData{$G=(X,U)$ such that $G^{tc}$ is an order.}
%\KwResult{$G’=(X,V)$ with $V\subseteq U$ such that $G’^{tc}$ is an interval order.}
\caption{\textsf{ROUTING} (node $src$, node $dst$, level $lowestLevel$)}

Search for node $dst$ using standard skip graph search algorithm in the subgraph rooted by the linked list at level $lowestLevel$ that contains $src$. Staring from the level $H_t - 1$, search goes down to lower levels $H_t -1, H_t - 2, \dots$, until the destination $v$ is found. Search ends at level $lowestLevel$. \ForAll {levels $d = H_t -1, H_t - 2, \dots lowestLevel$ in skip graph}{

	
	\If{destination $dst$ is found}{ establish connection between $src$ and $dst$ and \textbf{terminate} the subroutine. }
	
	\If{$L^{src}_d \neq 0$}{ The node currently processing the search at level $d$ finds a nearest node $w$ (must be found in $a$ rounds due to the a-balance property) in the sibling subgraph at level $L^{src}_d$. Node $w$ parallelly and recursively initiates \textsf{ROUTING} ($src$, $dst$, $d$).  }

}
\end{algorithm}


When the routing is done, $v$ records $\alpha$ and share $\alpha$ with $u$. Then both nodes $u$ and $v$ broadcast a transformation notification to all nodes in $l_\alpha$.  The notification includes all $H_t$ timestamps, group-ids and membership vectors of node $u$ and $v$. All nodes $x \in l_\alpha$ set $L^x_{\alpha+1} = L^x_{\alpha+2}, \dots, L^x_{H_t} = 0$.


All nodes $x \in l_\alpha$ set $L^x_{\alpha+1} = L^x_{\alpha+2}, \dots, L^x_{H_t} = 0$.

Let $lowest(T^y_d)$ be the lowest (earliest) timestamp at level $d$ among all nodes $x$ s.t. $G^x_d = G^y_d$ (i.e. all nodes in the group of $y$ at level $d$). All $lowest(T^u_d)$s for $d = \alpha, \alpha +1, ... , H_t - 1$ are computed using the skip list headed by node $u$, and all $lowest(T^v_d)$s for $d = \alpha, \alpha +1, ... , H_t - 1$ are computed using the skip list headed by node $v$. To compute $lowest(T^u_d)$, all nodes $x \in l_\alpha$ with $G^x_\alpha = G^u_\alpha$ linearly forward their level $\alpha$ timestamp $T^x_\alpha$ to their nearest right neighbor that stepped up to level $\alpha + 1$ in the skip list headed by node $u$. These forward actions take place using the level $\alpha$ links. A detailed description of a similar linear forwarding is presented in section \ref{sec:amf}. A node at level $\alpha + 1$ can receive at most $a$ timestamps from level $\alpha$ due to the a-balance property. These nodes at level $\alpha + 1$ locally find the lowest timestamp among the timestamps received and linearly forward the lowest timestamp with their level $\alpha+1$ timestamps $T^x_{\alpha+1}$ to the nearest right neighbor that stepped up to level $\alpha + 2$ in the skip list headed by node $u$. Thus, a node at level $\alpha + 2$ can receive at most $a$ level $\alpha$ and level $\alpha + 1$ timestamps. These nodes compute two lowest timestamps, one for the level $\alpha$ and another for the level $\alpha + 1$, and linearly forward these two lowest timestamps with their level $\alpha + 2$ timestamps $T^x_{\alpha+2}$ to their nearest right neighbor at level $\alpha + 3$ of the skip list headed by node $u$. This way after at most $a(H_t - \alpha)$ rounds node $u$ have all $lowest(T^u_d)$ for $d = \alpha, \alpha +1, ... , H_t - 1$. Similarly and parallelly, all $lowest(T^v_d)$ for $d = \alpha, \alpha +1, ... , H_t - 1$ are computed by using the skip list headed by node $v$. Node $u$ and $v$ broadcast all these lowest times to all nodes in $l_\alpha$.



(Rule for nodes in the same group of either communicating nodes at level $\alpha$). All nodes $x \in l_\alpha, x \neq u, x \neq v, G^x_\alpha = G^u_\alpha$ assign their priority based on the longest common prefix between their membership vector and the membership vector of node $u$. Each such node $x$ sets $P(x) = min(T^x_c, lowest(T^u_c))$ where $c$ is the size of longest common prefix between $m(u)$ and $m(x)$. Similarly, All nodes $x \in l_\alpha, x \neq u, x \neq v, G^x_\alpha = G^v_\alpha$ assign $P(x) = min(T^x_c, lowest(T^v_c))$ where $c$ is the size of longest common prefix between $m(v)$ and $m(x)$.



\fi
